On Fairness of Medical Image Classification with Multiple Sensitive Attributes via Learning Orthogonal Representations

Mitigating the discrimination of machine learning models has gained increasing attention in medical image analysis. However, rare works focus on fair treatments for patients with multiple sensitive demographic ones, which is a crucial yet challenging problem for real-world clinical applications. In this paper, we propose a novel method for fair representation learning with respect to multi-sensitive attributes. We pursue the independence between target and multi-sensitive representations by achieving orthogonality in the representation space. Concretely, we enforce the column space orthogonality by keeping target information on the complement of a low-rank sensitive space. Furthermore, in the row space, we encourage feature dimensions between target and sensitive representations to be orthogonal. The effectiveness of the proposed method is demonstrated with extensive experiments on the CheXpert dataset. To our best knowledge, this is the first work to mitigate unfairness with respect to multiple sensitive attributes in the field of medical imaging.

==> sections/02-Analysis.tex <==
\section{Analysis}


==> sections/05-Discussion.tex <==
\section{Discussion}



==> sections/old_method.tex <==
\section{Old Method}
Considering a fair classification setup where the inputs $x \in \mathcal{X} \subset \R^d$ , labels $y \in \mathcal{Y} = \{0, 1, ... , c\}$, where $c$ is the number of classes, The conjunction, i.e., Cartesian product, of $m$ binary sensitive attributes $A\in\prod_{i}A_i$ where the $i$-th sensitive attribute $A_i=\{0,1\}$, and prediction score $R=f(x)$ of the classification model $f$ that predicts a label $y$ given an input $x$.
%$R \in [0,1]$. 
\XL{from here to the end of the paragraph, I don't think it is preliminary} We first defined two separated encoders $\phi_T$ and $\phi_S$ to avoid the introducing of sensitive label information into target encoder during training. The two encoders then map input $x$ to two orthogonal low-dimensional representations and normalied into $Z_T \in \R^{B\times D}$ ,  $Z_S \in \R^{B\times D}$ respectively, where $B$ is the batch size, $D$ are dimensions of the representation. 
\subsubsection{Group Fairness} \XL{Again, here I dont think $y \in \{0,1\}$ is necessary}
The concept of fairness has been studied in many fields but no general definition of fairness exists~\cite{saxena2019per}. This work, we mainly focus on group fairness which considers within or between group fairness ({\it e.g.}, young vs. old and young women vs. old men, respectively). We aims at achieving equalized odds disparity(ED) $P(R|A=1,Y=y) = P(R|A=0,Y=y)$ for $y \in \{0,1\}$. Given the difficulty of optimizing the independency constraints, we use the relaxed metric:
$$max_{y\in\{0,1\}} |P(R|A=1,Y=y) - P(R|A=0,Y=y)|$$
\XL{Check your $A$ here, misalignment!}
Recent studies~\cite{dullerud2022fairness,sarhan2020fairness,park2021learning} also used this metric, however, they decorrelate the whole feature pair and achieving the orthogonality $R\perp A$ \XL{After noting $R=f(x)$, I think this is correct. You need to add problem formulation and show the linkage to orthogonality}which ignored the possible correlations between $A$ and $Y$. \XL{who did this poor writing??? why starting with \ie and pls see how I used \ie} \DWL{me...}\ie, when sensitive groups have various distributions for $Y$. Ignoring these dependencies could harm the learning of predictor\cite{chuang2021fair}. Hence, we consider the orthogonality with each class $R \perp A | Y$.

\XL{You may want a paragraph for problem formulation}


\subsubsection{Sensitive Representation Space}\label{sep}
\XL{I did not get he purpose of this paragraph, especially you put it under preliminary}
Shared encoder may meets the leakage of sensitive information during training, so Sarhan \XL{and please note how I used \etal} \textit{et.al}~\cite{sarhan2020fairness} freezed the the backpropogation when training with sensitive label, however, it cannot well train the sensitive task. Recently, Dullerud  \textit{et.al}~\cite{dullerud2022fairness} reduced the learning rate when train sensitive task, however, it will still introduce sensitive label information. To overcome the problem, we used a seperated network $\phi_S$ to produced $Z_S$. In this way, we can pre-train the $\phi_S$ to produce high quality multi-sensitive representations. In our case, we select the pretrained model that can achieve good and balanced performance on every sensitive class to produce representations. We plot the resulting Representation with t-SNE in Figure \ref{fig:tsne}.
% \begin{align}
%     L_{corr} &= mean[(\phi^{targ}(X)- \mu^{targ})^{T}  (\phi^{SA}(X)- \mu^{SA})]\\
%           & = \frac{1}{N^2}\sum^N_{i=1}\sum^N_{j=1} \overline{\phi^{targ}(X)}_{(:,i)}^{T} \overline{\phi^{targ}(X)}_{(:,j)} 
% \end{align}


% feature space orthogonal, feature is not aligned, so require orthogonal within every feature vector, which naturally obtain the covariance, This it still deserves to design a better statistical independence loss for the hard multi-sensitive attributes setting. Let $\phi^{targ}(X)$ and $\phi^{SA}(X) \in R^{B\times D}$ denote the intermediate feature map, where $B$ is the batch size, $D$ are dimensions of the feature map.


% Inspired by the popular whitening~\cite{choi2021robustnet,huang2018decorrelated} in disentanglement and domain adaptation

\subsection{Sample Space Orthogonality}\label{sta}
\XL{Move this section after feature orthogonality}
\XL{Here is a gap...how sample space orthogonality is related to your problem formulation.}
In this section, we propose the Sample Space Orthogonality, which not only enhanced the multi-sensitive fairness but also improve the efficiency in finite samples. 
\subsubsection{Sample Space Fairness} Current methods~\cite{dullerud2022fairness,park2021learning,zhu2021learning} reduce mutual information between sensitive and target representations, \XL{One?} a shortcome is they are only sample-wise methods, which is not sufficient for the complex multi-sensitive fairness \XL{I did not get this sentence}. As a result \XL{wrong phrase used here}, we proposed to achieve sample space fairness to encourage every sample space bases being orthogonal to each other. Taking the normalized intermediate feature $Z_T, Z_S$, we say $Z_T^i \in R^{B\times1}$ is the $i$th target sample bases, we wish it to be orthogonal to the sample bases from sensitive representation $Z_S$. As a result, our stronger sample space orthogonal loss will be:
\XL{Please avoid double sub and super-scripts}
\begin{align}
    L_{sorth} &= \mathbb{E}[||Z_{T}- \mu_{T})^{\top}  (Z_{S}- \mu_{S})||_2]\\
          & = \frac{1}{D^2}\sum^D_{i=1}\sum^D_{j=1} ||\hat{Z}^i_{T}^{\top} \hat{Z}^j_{S}||
\end{align}
Where $\mu = \frac{1}{D} 1\cdot Z \in R^{1\times D}$. It is notable that our loss will naturally become the covariance loss that computed on feature space. With this loss, we can achieve a better and more stable multi-sensitive fairness.
\subsubsection{Learning Efficiency}  Here we compare the rademacher complexity between $\mathcal{F}_{L_2}$ and  $\mathcal{F}_{L_2,sorth}$.  Considering sample space orthogonal constraint restricts the projection of the weights $w$ onto $\Delta := sorth(X,Z_S) = Cov(X,Z_S) = \sum^{D}_{i=1}Cov(X,Z_S^{i})$ and $w_{\perp}:= \Pi w$ as the projection, which can be regarded as irrelevant space of $X$. Assume, $x_{\perp} := \Pi x$, $x_{||} := (\mathcal{I} - \Pi) x$ and $sup_{x_{||}}||x_{||}||_2 \leq B_{||}$,$sup_{x_{\perp}}||x_{\perp}||_2 \leq B_{\perp}$. We can directly compare our results with \cite{makar2022causally}, since $Z_S^{i}$ is one dimensional and $\Delta$ is a vector. Due to the limited space,
we only present an informal statement here. The formal
statement can be found in Appendix \ref{effi}.\\
\XL{Notations here are poorly defined}
\textbf{Proposition 1} Let $f(x) = \delta(\phi(x)) = \delta(w^{\top}x)$ be a function contained in $FL_{2,cov}$ Then, $||w_{\perp}|| \leq \frac{\gamma}{\Delta}$. and 
\begin{align}
    \mathcal{R}(F_{L_2}) \leq \frac{C\sqrt{B^2_{||}+B^2_{\perp}}}{\sqrt{n}}, \mathcal{R}(F_{L_2,cov}) \leq \frac{C\cdot B_{||}+\gamma \frac{B_{\perp}}{||\Delta||}}{\sqrt{n}}
\end{align}

Where n is the number of data. As we can see, our regularization suppressed the rachemacher complexity on the sensitive related parameters, which helps the learning efficiency.

% Thus, enforcing the diagonal of the covariance matrix to be zero is just the mutual information loss, The off-diagonal of the covariance matrix helps a better statistical independence. In addition, Lemma 1 gives us a theoretically proof of the statistical independence that achieved by reducing covariance.\\
% {\bf Lemma 1:}~\cite{adeli2021representation} \textit{Given random variables $F,B,\hat{B}$ with finite second moment, $B$ is statistical mean independent of $F \Leftrightarrow$ for any arbitrary mapping $\phi,s.t. \hat{B}=\phi(F),cov(B,\hat{B})=0$.}\\

\subsection{Feature Space Orthogonality}\label{ortho}\todo{Re-wright feature space orthogonality here.}
In this section, we wish to extract multi-sensitive feature bases $\mathcal{B}$ and achieve feature space orthogonality by reducing projected target information on sensitive bases. Challenge are 1) Obtain a low rank matrix that could well capture the major information. 2) Efficiently extract sensitive feature bases.  To achieve first goal, we proposes to encode multi-sensitive information into a single representation and construct feature basis by decomposing the sensitive representation with singular value decomposition (SVD).  To achieve the second goal, we proposed two bases extraction schema based on SVD: Direct Extraction and Basis Accumulation.
\XL{Connection between this two paragraph can be enhanced}
\subsubsection{Direct Extraction} aims at obtaining subspaces that could well represent the batch statistical information, Specifically, the SVD is applied to the centered sensitive representations $Z_S ^{\top} = U \Sigma V$, \XL{since we use $Z \in \R^{d\times n}$ now, you don't need transpose here anymore} where $U = [u_1, ... , u_D] \in 
R^{D\times D}$ is an orthogonal matrix with left singular vector $u_i \in R^{D}$, $V = [v_1, ... , v_B] \in \R^{B\times B}$ is an orthogonal matrix with left singular vector $v_i \in R^{B}$, and $\Sigma \in R^{D\times B}$ is a rectangular diagonal matrix with descending non-negative singular values $\{\delta_i\}_{i=1}^{min\{B,D\}}$. In this paper, we call $U \in R^{B\times B}$ as space basis which reduces the data dimension.


% a novel approach to accumulate batch information into a global one by 1) constructing data basis by decomposing the batch feature with singular value decomposition (SVD) 2) accumulate important basis and use the most related previous basis to calculate statistical independence for current batch. This paper only extract the global information for multi-sensitive attributes for efficiency and easier optimization.

\subsubsection{Basis Accumulation} aspires to aggregate important representative bases into a global statistics to remove the influence from multi-sensitive attributes. For clearly, we define training iteration as $t \in [1,,2,...,T]$, then the $\mathcal{C}_s^t$ as the cache set at iteration t whose maximum size is $s$, the multi-sensitive representation matrix at iteration $t$ as $R^t$, the decomposed orthogonal matrix at iteration $t$ as $\mathcal{B}^t$ and singular vector as $b^t_i$, where $i \in B$ for data basis and $i \in D$ for space basis. We then designed following procedures to achieve the ultimate goal:
\begin{itemize}
    \item For $t = 1$, all the bases $\mathcal{B}^1$ will be directly applied to remove multi-sensitive attributes with orthogonal loss $L_{gorth}$, then inserted into $\mathcal{C}_s^1$ for future calculation.
    \item For $t \in [2,T]$, Since the previous information set $\mathcal{C}_s^{t-1}$ could include important bases for current batch. Therefore, for each basis in $\mathcal{C}_s^{t-1}$, we compute its corresponding eigenvalue on $R^t(R^t)'$ as $\delta^t_i=(b^t_i)'R^t(R^t)'b^t_i$ and obtained singular values $\Delta^t_c$. Then we use SVD to decompose $R^t$ to obtain bases $\mathcal{B}^t$ and their corresponding singular values $\Delta^t$. After that, we select top bases $B^t_{best}$ according to their singular values by concatenating $\Delta^t$ and $\Delta^t_c$ and sort in descending order. Finally, $B^t_{best}$ is added into $\mathcal{C}_s^{t-1}$ and pop the oldest one if exceed the maximum size.
    \item At each iteration $t \in [2,T]$, we calculate the orthogonal loss $L_{orth}$ with the $B^t_{best}$. In this way, our loss removed multi-sensitive attributes influence from a global aspective.
\end{itemize}
where the the global orthogonal loss $L_{gcorr}$ is defined as:
\begin{align}
    L_{orth} &= \mathbb{E}[\phi^{targ}(X) \times B_{best}] 
\end{align}
By reducing the target information that projected on multi-sensitive bases, we achieved the orthogonal between target representation and multi-sensitive attribubtes representation.
